Relational Network for Skeleton-Based Action Recognition

With the fast development of effective and low-cost human skeleton capture systems, skeleton-based action recognition has attracted much attention recently. Most existing methods use Convolutional Neural Network (CNN) and Recurrent Neural Network (RNN) to extract spatio-temporal information embedded in the skeleton sequences for action recognition. However, these approaches are limited in the ability of relational modeling in a single skeleton, due to the loss of important structural information when converting the raw skeleton data to adapt to the input format of CNN or RNN. In this paper, we propose an Attentional Recurrent Relational Network-LSTM (ARRN-LSTM) to simultaneously model spatial configurations and temporal dynamics in skeletons for action recognition. We introduce the Recurrent Relational Network to learn the spatial features in a single skeleton, followed by a multi-layer LSTM to learn the temporal features in the skeleton sequences. Between the two modules, we design an adaptive attentional module to focus attention on the most discriminative parts in the single skeleton. To exploit the complementarity from different geometries in the skeleton for sufficient relational modeling, we design a two-stream architecture to learn the structural features among joints and lines simultaneously. Extensive experiments are conducted on several popular skeleton datasets and the results show that the proposed approach achieves better results than most mainstream methods.

==> icme2019template <==

%[1] Microsoft kinect sensor and its effect
@article{zhang2012microsoft,
  title={Microsoft kinect sensor and its effect},
  author={Zhang, Zhengyou},
  journal={IEEE Multimedia},
  volume={19},
  number={2},
  pages={4--10},
  year={2012},
  publisher={IEEE}
}
%[2]
@article{IntelRealSense,
  title={Intel RealSense. https://software.intel.com/en-us/realsense.1},
  }

%[3] Real-time human pose recognition in parts from single depth images
@inproceedings{shotton2011real,
  title={Real-time human pose recognition in parts from single depth images},
  author={Shotton, Jamie and Fitzgibbon, Andrew and Cook, Mat and Sharp, Toby and Finocchio, Mark and Moore, Richard and Kipman, Alex and Blake, Andrew},
  booktitle={CVPR},
  pages={1297--1304},
  year={2011},
  organization={IEEE}
}
%[3.5] 3d skeleton-based human action classification: a survey
@article{presti20163d,
  title={3D skeleton-based human action classification: A survey},
  author={Presti, Liliana Lo and La Cascia, Marco},
  journal={Pattern Recognition},
  volume={53},
  pages={130--147},
  year={2016},
  publisher={Elsevier}
}
%[4] Mining actionlet ensemble for action recognition with depth cameras
@inproceedings{wang2012mining,
  title={Mining actionlet ensemble for action recognition with depth cameras},
  author={Wang, Jiang and Liu, Zicheng and Wu, Ying and Yuan, Junsong},
  booktitle={CVPR},
  pages={1290--1297},
  year={2012},
  organization={IEEE}
}
%[5] Bio-inspired dynamic 3d discriminative skeletal features for human action recognition

%[6] Human actiion recognition using a temporal hierarchy of covariance descriptors on 3D joint locations


%[7] Joint angles similarities and HOG2 for action recognition
@inproceedings{ohn2013joint,
  title={Joint angles similarities and HOG2 for action recognition},
  author={Ohn-Bar, Eshed and Trivedi, Mohan M},
  booktitle={CVPRW},
  pages={465--470},
  year={2013},
  organization={IEEE}
}
%[8] Human action recognition by representing 3d skeletons as points in a lie group
@inproceedings{vemulapalli2014human,
  title={Human action recognition by representing 3d skeletons as points in a lie group},
  author={Vemulapalli, Raviteja and Arrate, Felipe and Chellappa, Rama},
  booktitle={CVPR},
  pages={588--595},
  year={2014},
  organization={IEEE}
}
%[9] Mining actionlet ensemble for action recognition with depth cameras
@inproceedings{wang2012mining,
  title={Mining actionlet ensemble for action recognition with depth cameras},
  author={Wang, Jiang and Liu, Zicheng and Wu, Ying and Yuan, Junsong},
  booktitle={CVPR},
  pages={1290--1297},
  year={2012},
  organization={IEEE}
}
%[10] The moving pose: an efficient 3d kenematics descriptor for low-latency action recognition and detection

@inproceedings{zanfir2013moving,
  title={The moving pose: An efficient 3d kinematics descriptor for low-latency action recognition and detection},
  author={Zanfir, Mihai and Leordeanu, Marius and Sminchisescu, Cristian},
  booktitle={ICCV},
  pages={2752--2759},
  year={2013},
  organization={IEEE}
}
%[10.5] Mining mid-level features for action recognition based on effective skeleton representation

@inproceedings{wang2014mining,
  title={Mining mid-level features for action recognition based on effective skeleton representation},
  author={Wang, Pichao and Li, Wanqing and Ogunbona, Philip and Gao, Zhimin and Zhang, Hanling},
  booktitle={DlCTA},
  pages={1--8},
  year={2014},
  organization={IEEE}
}
%[19] Gradient-based learning applied to document recognition
@article{lecun1998gradient,
  title={Gradient-based learning applied to document recognition},
  author={LeCun, Yann and Bottou, L{\'e}on and Bengio, Yoshua and Haffner, Patrick},
  journal={Proceedings of the IEEE},
  volume={86},
  number={11},
  pages={2278--2324},
  year={1998},
  publisher={IEEE}
}
%[20] Generalization of back-propagation to recurrent neural network
@article{pineda1987generalization,
  title={Generalization of back-propagation to recurrent neural networks},
  author={Pineda, Fernando J},
  journal={Physical Review Letters},
  volume={59},
  number={19},
  pages={2229},
  year={1987},
  publisher={APS}
}
%[20.1] a simple neural network module for relational reasoning
@inproceedings{santoro2017simple,
  title={A simple neural network module for relational reasoning},
  author={Santoro, Adam and Raposo, David and Barrett, David G and Malinowski, Mateusz and Pascanu, Razvan and Battaglia, Peter and Lillicrap, Tim},
  booktitle={NIPS},
  pages={4974--4983},
  year={2017}
}
%[20.2] CLEVR: A Diagnostic Dataset for Compositional Language and Elementary Visual Reasoning
@inproceedings{johnson2017clevr,
  title={CLEVR: A diagnostic dataset for compositional language and elementary visual reasoning},
  author={Johnson, Justin and Hariharan, Bharath and van der Maaten, Laurens and Fei-Fei, Li and Zitnick, C Lawrence and Girshick, Ross},
  booktitle={CVPR},
  pages={1988--1997},
  year={2017},
  organization={IEEE}
}
%[20.3] recurrent relational networks for complex relational reasoning
@article{palm2017recurrent,
  title={Recurrent Relational Networks for Complex Relational Reasoning},
  author={Palm, Rasmus Berg and Paquet, Ulrich and Winther, Ole},
  journal={arXiv preprint arXiv:1711.08028},
  year={2017}
}

%[21] ImageNet Classification with Deep Convolutional Neural Networks
%@inproceedings{krizhevsky2012imagenet,
%  title={Imagenet classification with deep convolutional neural networks},
%  author={Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
%  booktitle={NIPS},
%  pages={1097--1105},
%  year={2012}
%}
%[23] deep learning based human action recognition: a survey
%@article{zhangdeep,
%  title={Deep Learning Based Human Action Recognition: A Survey},
%  author={Zhang, Zhimeng and Ma, Xin and Song, Rui and Rong, Xuewen and Tian, Xincheng and Tian, Guohui and Li, Yibin}
%}
%[24] Skeleton Optical Spectra Based Action recognition using convolutional neural network
@article{hou2016skeleton,
  title={Skeleton optical spectra based action recognition using convolutional neural networks},
  author={Hou, Yonghong and Li, Zhaoyang and Wang, Pichao and Li, Wanqing},
  journal={IEEE Transactions on Circuits and Systems for Video Technology},
  year={2016},
  publisher={IEEE}
}
%[25] action recognition based on joint trajectory maps using convolutional neural networks
@inproceedings{wang2016action,
  title={Action recognition based on joint trajectory maps using convolutional neural networks},
  author={Wang, Pichao and Li, Zhaoyang and Hou, Yonghong and Li, Wanqing},
  booktitle={ACMMM},
  pages={102--106},
  year={2016},
  organization={ACM}
}
%[26] Human action recognition using RGB-D sensor and deep convolutional neural networks
@inproceedings{imran2016human,
  title={Human action recognition using RGB-D sensor and deep convolutional neural networks},
  author={Imran, Javed and Kumar, Praveen},
  booktitle={ICACCI},
  pages={144--148},
  year={2016},
  organization={IEEE}
}
%[27] Two-stream 3d convolutional neural network for skeleton-based action recognition
@article{liu2017two,
  title={Two-Stream 3D Convolutional Neural Network for Skeleton-Based Action Recognition},
  author={Liu, Hong and Tu, Juanhui and Liu, Mengyuan},
  journal={arXiv preprint arXiv:1705.08106},
  year={2017}
}

%[28] SKELETON BASED ACTION RECOGNITION WITH CONVOLUTIONAL NEURAL NETWORK
@inproceedings{du2015skeleton,
  title={Skeleton based action recognition with convolutional neural network},
  author={Du, Yong and Fu, Yun and Wang, Liang},
  booktitle={ACPR},
  pages={579--583},
  year={2015},
  organization={IEEE}
}
%[29] skeleton based action recognition using translation-scale invariant image mapping and multi-scale deep CNN
@inproceedings{li2017skeleton,
  title={Skeleton based action recognition using translation-scale invariant image mapping and multi-scale deep CNN},
  author={Li, Bo and Dai, Yuchao and Cheng, Xuelian and Chen, Huahui and Lin, Yi and He, Mingyi},
  booktitle={ICMEW},
  pages={601--604},
  year={2017},
  organization={IEEE}
}
%[30] SKELETON-BASED ACTION RECOGNITION WITH CONVOLUTIONAL NEURAL NETWORKS
@inproceedings{du2015skeleton,
  title={Skeleton based action recognition with convolutional neural network},
  author={Du, Yong and Fu, Yun and Wang, Liang},
  booktitle={ACPR},
  pages={579--583},
  year={2015},
  organization={IEEE}
}
%[31] SkeletonNet: Mining Deep Part Features for 3-D Action Recognition
@article{ke2017skeletonnet,
  title={Skeletonnet: Mining deep part features for 3-d action recognition},
  author={Ke, Qiuhong and An, Senjian and Bennamoun, Mohammed and Sohel, Ferdous and Boussaid, Farid},
  journal={Signal Processing Letters},
  volume={24},
  number={6},
  pages={731--735},
  year={2017},
  publisher={IEEE}
}
%[32] Joint Distance maps based action recognition with convolutional neural networks
@article{li2017joint,
  title={Joint distance maps based action recognition with convolutional neural networks},
  author={Li, Chuankun and Hou, Yonghong and Wang, Pichao and Li, Wanqing},
  journal={Signal Processing Letters},
  volume={24},
  number={5},
  pages={624--628},
  year={2017},
  publisher={IEEE}
}
%33] A new representation of skeleton sequences for 3d action recognition
@inproceedings{ke2017new,
  title={A new representation of skeleton sequences for 3d action recognition},
  author={Ke, Qiuhong and Bennamoun, Mohammed and An, Senjian and Sohel, Ferdous and Boussaid, Farid},
  booktitle={CVPR},
  pages={4570--4579},
  year={2017},
  organization={IEEE}
}
%[34] investigate of different skeleton features for cnn-based 3d action recognition
@inproceedings{ding2017investigation,
  title={Investigation of different skeleton features for CNN-based 3D action recognition},
  author={Ding, Zewei and Wang, Pichao and Ogunbona, Philip O and Li, Wanqing},
  booktitle={ICMEW},
  pages={617--622},
  year={2017},
  organization={IEEE}
}
%[34.1]spatial Temporal graph convolutional network for skeleton-based action recognition
@article{yan2018spatial,
  title={Spatial Temporal Graph Convolutional Networks for Skeleton-Based Action Recognition},
  author={Yan, Sijie and Xiong, Yuanjun and Lin, Dahua},
  journal={arXiv preprint arXiv:1801.07455},
  year={2018}
}

%[35] Hierarchical Recurrent Neural Network for Skeleton Based Action Recognition
@inproceedings{du2015hierarchical,
  title={Hierarchical recurrent neural network for skeleton based action recognition},
  author={Du, Yong and Wang, Wei and Wang, Liang},
  booktitle={CVPR},
  pages={1110--1118},
  year={2015},
  organization={IEEE}
}
%[36] Modeling temporal dynamics and spatial configurations of actions using two-stream recurrent neural network
@inproceedings{wang2017modeling,
  title={Modeling temporal dynamics and spatial configurations of actions using two-stream recurrent neural networks},
  author={Wang, Hongsong and Wang, Liang},
  booktitle={CVPR},
  year={2017},
  organization={IEEE}
}
%[37] Co-occurrence Feature learning for skeleton based action recognition using regularized deep lstm networks
@inproceedings{zhu2016co,
  title={Co-Occurrence Feature Learning for Skeleton Based Action Recognition Using Regularized Deep LSTM Networks.},
  author={Zhu, Wentao and Lan, Cuiling and Xing, Junliang and Zeng, Wenjun and Li, Yanghao and Shen, Li and Xie, Xiaohui and others},
  booktitle={AAAI},
  volume={2},
  pages={8},
  year={2016}
}
%[38] Ntu rgb+d: a large scale dataset for 3d human activity analysis
@article{shahroudy2016ntu,
  title={NTU RGB+ D: A large scale dataset for 3D human activity analysis},
  author={Shahroudy, Amir and Liu, Jun and Ng, Tian-Tsong and Wang, Gang},
  journal={arXiv preprint arXiv:1604.02808},
  year={2016}
}

%[39] spatio-temporal lstm with trust gates for 3d human action recognition
@inproceedings{liu2016spatio,
  title={Spatio-temporal lstm with trust gates for 3d human action recognition},
  author={Liu, Jun and Shahroudy, Amir and Xu, Dong and Wang, Gang},
  booktitle={ECCV},
  pages={816--833},
  year={2016},
  organization={Springer}
}
%[40] skeleton-based action recognition using lstm and cnn
%@inproceedings{li2017skeleton,
%  title={Skeleton-based action recognition using LSTM and CNN},
%  author={Li, Chuankun and Wang, Pichao and Wang, Shuang and Hou, Yonghong and Li, Wanqing},
%  booktitle={ICMEW},
%  pages={585--590},
%  year={2017},
%  organization={IEEE}
%}
\end{thebibliography}

@inproceedings{li22017skeleton,
  title={Skeleton-based action recognition with convolutional neural networks},
  author={Li, Chao and Zhong, Qiaoyong and Xie, Di and Pu, Shiliang},
  booktitle={ICMEW},
  pages={597--600},
  year={2017},
  organization={IEEE}
}

@inproceedings{paszke2017automatic,
  title={Automatic differentiation in PyTorch},
  author={Paszke, Adam and Gross, Sam and Chintala, Soumith and Chanan, Gregory and Yang, Edward and DeVito, Zachary and Lin, Zeming and Desmaison, Alban and Antiga, Luca and Lerer, Adam},
  booktitle={NIPSW},
  year={2017}
}


}
%[41] Jointly learning heterogeneous features for rgb-d activity recognition
@inproceedings{hu2015jointly,
  title={Jointly learning heterogeneous features for RGB-D activity recognition},
  author={Hu, Jian-Fang and Zheng, Wei-Shi and Lai, Jianhuang and Zhang, Jianguo},
  booktitle={CVPR},
  pages={5344--5352},
  year={2015},
  organization={IEEE}
}
%[45] an end-to-end spatio-temporal attention model for human action recognition from skeleton data
@inproceedings{song2017end,
  title={An End-to-End Spatio-Temporal Attention Model for Human Action Recognition from Skeleton Data.},
  author={Song, Sijie and Lan, Cuiling and Xing, Junliang and Zeng, Wenjun and Liu, Jiaying},
  booktitle={AAAI},
  volume={1},
  number={2},
  pages={7},
  year={2017}
}
%[46] view adaptive recurrent neural networks for high performance human action recognition from skeleton data
@inproceedings{zhang2017view,
  title={View adaptive recurrent neural networks for high performance human action recognition from skeleton data},
  author={Zhang, Pengfei and Lan, Cuiling and Xing, Junliang and Zeng, Wenjun and Xue, Jianru and Zheng, Nanning},
  booktitle={ICCV},
  pages={2136-2145},
  year={2017},
  organization={IEEE}
}
%[47] A new representation of skeleton sequences for 3d action recognition
@inproceedings{ke2017new,
  title={A new representation of skeleton sequences for 3d action recognition},
  author={Ke, Qiuhong and Bennamoun, Mohammed and An, Senjian and Sohel, Ferdous and Boussaid, Farid},
  booktitle={CVPR},
  pages={4570--4579},
  year={2017},
  organization={IEEE}
}

@inproceedings{seidenari2013recognizing,
  title={Recognizing actions from depth cameras as weakly aligned multi-part bag-of-poses},
  author={Seidenari, Lorenzo and Varano, Vincenzo and Berretti, Stefano and Del Bimbo, Alberto and Pala, Pietro},
  booktitle={CVPRW},
  pages={479--485},
  year={2013},
  organization={IEEE}
}

@article{devanne20153,
  title={3-d human action recognition by shape analysis of motion trajectories on riemannian manifold},
  author={Devanne, Maxime and Wannous, Hazem and Berretti, Stefano and Pala, Pietro and Daoudi, Mohamed and Del Bimbo, Alberto},
  journal={IEEE Transactions on Cybernetics},
  volume={45},
  number={7},
  pages={1340--1352},
  year={2015},
  publisher={IEEE}
}

@inproceedings{vemulapalli2014human,
  title={Human action recognition by representing 3d skeletons as points in a lie group},
  author={Vemulapalli, Raviteja and Arrate, Felipe and Chellappa, Rama},
  booktitle={CVPR},
  pages={588--595},
  year={2014}
}

@inproceedings{wang2016graph,
  title={Graph based skeleton motion representation and similarity measurement for action recognition},
  author={Wang, Pei and Yuan, Chunfeng and Hu, Weiming and Li, Bing and Zhang, Yanning},
  booktitle={ECCV},
  pages={370--385},
  year={2016},
  organization={Springer}
}



@article{li2018spatio,
  title={Spatio-Temporal Graph Convolution for Skeleton Based Action Recognition},
  author={Li, Chaolong and Cui, Zhen and Zheng, Wenming and Xu, Chunyan and Yang, Jian},
  journal={arXiv:1802.09834},
  year={2018}
}

@inproceedings{koniusz2016tensor,
  title={Tensor representations via kernel linearization for action recognition from 3D skeletons},
  author={Koniusz, Piotr and Cherian, Anoop and Porikli, Fatih},
  booktitle={ECCV},
  pages={37--53},
  year={2016},
  organization={Springer}
}

@article{weng2018discriminative,
  title={Discriminative Spatio-Temporal Pattern Discovery for 3D Action Recognition},
  author={Weng, Junwu and Weng, Chaoqun and Yuan, Junsong and Liu, Zicheng},
  journal={IEEE Transactions on Circuits and Systems for Video Technology},
  year={2018},
  publisher={IEEE}
}

@inproceedings{du2015hierarchical,
  title={Hierarchical recurrent neural network for skeleton based action recognition},
  author={Du, Yong and Wang, Wei and Wang, Liang},
  booktitle={CVPR},
  pages={1110--1118},
  year={2015},
  organization={IEEE}
}

